ALT: Boosting Deep Learning Performance by Breaking the Wall between Graph and Operator Level Optimizations

Deep learning models rely on highly optimized tensor libraries for efficient inference on heterogeneous hardware. Current deep compilers typically predetermine layouts of tensors and then optimize loops of operators. However, such unidirectional and one-off workflow strictly separates graph-level optimization and operator-level optimization into different system layers, missing opportunities for unified tuning. This paper proposes ALT, a compiler that performs joint graph- and operator-level optimizations for deep models. ALT provides a generic transformation module to manipulate layouts and loops with easy-to-use primitive functions. ALT further integrates an auto-tuning module that jointly optimizes graph-level data layouts and operator-level loops while guaranteeing efficiency. Experimental results show that ALT significantly outperforms state-of-the-art compilers (e.g., Ansor) in terms of both single operator performance (e.g., 1.5x speedup on average) and end-to-end inference performance (e.g., 1.4x speedup on average).

==> secs/experim.tex <==
% \vspace{-0.18in}
% \vspace{-0.03in}
\presec\section{Evaluation}
% \postsec
% \vspace{0.01in}
%In this section, we will evaluate \sys to illustrate its performance, and verify the effectiveness of our proposed techniques.
%
%In this section, we evaluate \sys to verify its effectiveness. 
%During evaluating \sys, we want to answer the following questions: (1) how does \sys perform compared with state-of-the-art compilers or frameworks; (2) where is the performance gain from; (3) how fast is the search; (4) how do we explain the optimized layouts.
% \vspace{-0.1in}
%\presub\subsection{Experimentation Setup}\postsub
% \vspace{-0.02in}
In this section, we evaluate \sys on various hardware platforms, including 40-core Intel Xeon Gold 6248 CPU@2.5GHz (443GB memory), NVIDIA Tesla V100 (CUDA v11.0), and Kirin 990 SoC (Android v10). We compare \sys with state-of-the-art frameworks and compilers: Torch (v1.7) \cite{paszke2019pytorch}, AutoTVM (v0.8dev1) \cite{chen2018learning}, FlexTensor \cite{zheng2020flextensor}, and Ansor \cite{zheng2020ansor}.
% 这里不用讲was evaluated by using the ... library ...吧
Torch is a reference point for vendor libraries, which was evaluated by using MKL-DNN library \cite{mkldnn} for Intel CPU, cuDNN (v8.0.4) library \cite{chetlur2014cudnn} for NVIDIA GPU, and XNNPACK library \cite{xnnpack} for ARM CPU. AutoTVM, FlexTensor, and Ansor are three widely used auto-tuning frameworks.
%It is notable that AutoTVM and Ansor have integrated NeoCPU \cite{liu2019optimizing}. 
Besides, Ansor outperforms Tensorflow Lite \cite{abadi2016tensorflow} and other hardware-specific compilers \cite{liu2019optimizing, zheng2020ansor} such as OpenVINO \cite{openvino} and TensorRT \cite{tensorrt}. Thus, we do not include them as baselines here.
%For all measurements, we obtained the results by averaging 100 on-device execution trials. 

For \sys, if not specified, we use one-level layout tiling templates for layout space building. For loop space exploration, we set the sampling batch size and the episode length to 128, 
% 这有点转圈说，而且它们重要吗？不重要放后面，放在这里留不下什么印象
and measure the top-8 points predicted by the cost model on the target hardware. In addition, we take the total number of such on-device measurements as a metric of the search budget for all auto-tuning methods. Thus, a batch or an episode of points in \sys will cost a budget of 8.

% \vspace{-0.03in}
\subsection{Single Operator Benchmark}
%\postsub
% \vspace{-0.01in}
\label{subsec:single_op_bench}


\begin{figure*}
	\centering
	\subfloat[Single Operator on Intel CPU.]{\label{subfig:exprim_op_llvm}{\includegraphics[width=0.33\textwidth]{imgs/single_op_cpu_arxiv.pdf}}}\hfill
	% \\
	\subfloat[Single Operator on NVIDIA GPU.]{\label{subfig:exprim_op_cuda}{\includegraphics[width=0.33\textwidth]{imgs/single_op_gpu_arxiv.pdf}}}\hfill
	% \\
	\subfloat[Single Operator on ARM CPU.]{\label{subfig:exprim_op_android}{\includegraphics[width=0.33\textwidth]{imgs/single_op_android_arxiv.pdf}}}\hfill
	\vspace{-0.05in}
	\caption{Single operator performance.}
	\label{fig:exprim_op}
	\vspace{-0.13in}
\end{figure*}


\begin{figure}
	\centering
	% \vspace{-0.05in}
	\centering
	\subfloat[Network on Intel CPU.]{\label{subfig:exprim_network_llvm}{\includegraphics[width=0.455\textwidth]{imgs/network_cpu_arxiv.pdf}}}\hfill
	\\
	% \vspace{-0.05in}
	\centering
	\subfloat[Network on NVIDIA GPU.]{\label{subfig:exprim_network_cuda}{\includegraphics[width=0.455\textwidth]{imgs/network_gpu_arxiv.pdf}}}\hfill
	\\
	\subfloat[Network on ARM CPU.]{\label{subfig:exprim_network_android}{\includegraphics[width=0.455\textwidth]{imgs/network_android_arxiv.pdf}}}\hfill
	\\
	\vspace{-0.05in}
	\caption{End-to-end inference performance.}
	\label{fig:exprim_network}
	\vspace{-0.15in}
\end{figure}

%\sys can be used to optimize single operators with little human effort. 
% 干掉？如果要说就好好说，否则会起到坏印象， for some operators
%\textcolor{red}{For practitioners, the generated program for a single operator can be directly integrated into applications. }
We first present the results on single operators. 
We consider 9 operators, including C2D, Group-wise C2D (GRP), Depth-wise C2D (DEP), Dilated C2D (DIL), 3-D convolution (C3D), 1-D convolution (C1D), GMM, Transposed C2D (T2D), Transposed C3D (T3D). Each operator is evaluated using 10 random configurations with different batch sizes, kernel sizes, etc. For instance, the value of batch size is selected from $[1, 16]$, and the number of input channels is uniformly sampled from $[3, 16, 32, 64, 512, 960, 1280]$. We generate 90 test cases for each device. The result is normalized based on the geometric mean of speedups over the worst latency of each test case. For C1D, C2D/T2D, and C3D/T3D and their variants, we test $NOW/NWO$ for C1D, $NOHW/NHWO$ for C2D/T2D, and $NODHW/NDHWO$ ($D$ is the depth dimension) for C3D/T3D and report the best for baselines except Torch (it only supports $NOW, NOHW, NODHW$). We set the search budget to 1000 for all auto-tuning methods, which is suggested by Ansor. For \sys, the budget for the joint stage and the loop-only stage is 300 and 700 respectively.

% \cref{fig:exprim_op} demonstrates the results and the standard error for ten cases of each operator for \sys.
As shown in \cref{subfig:exprim_op_llvm}, on Intel CPU \sys achieves $9.5\times$, $9.9\times$, $9.8\times$, and $1.6\times$ speedups in comparison with Torch, AutoTVM, FlexTensor, and Ansor respectively. Among all operators, DIL and DEP have lower operational intensity (the ratio of the number of computational instructions to the number of memory access instructions), and thus they are more likely to be memory-bound. For DIL and DEP, \sys outperforms other baselines with a large margin because layout tuning can effectively reduce memory accessing overheads. Even for operators that are typically compute-bound, \textit{e.g.}, C2D and C3D, \sys still achieves notable speedups. This is because the operational intensity depends on tensor shapes. \sys can tailor the tensor layouts toward each specific shape and hardware platform.
% In summary, \sys achieves average $9.1\times$, $8.8\times$, $9.0\times$, and $1.5\times$ speedup ratio compared with Torch, AutoTVM, FlexTensor, and Ansor, respectively, on Intel CPU (\cref{subfig:exprim_op_llvm}). 
%For the C2D operator which is often involved in benchmarks, the backends of Torch (MKL-DNN and cuDNN) put many efforts to its optimization especially the $3\times3$ kernels, thereby outperforming auto-tuning frameworks like AutoTVM and FlexTensor. However, Ansor exploits multiple templates which implies a much larger search space, but can still outperform manually-tuned libraries. On the other hand, since \sys integrates both layout and loop transformations, we can achieve an $1.3\times$ speedup compared with Ansor. 
%For all operators except C3D, \sys can outperform all baselines, often with a large margin. As for the C3D operator, Torch performs better than others on Intel CPU. However, \sys can still achieve comparable performance. We attribute the reason to the very high arithmetic intensity of C3D, and layout optimization can hardly be helpful in such cases. By contrast, \sys often achieves favorable speedups on operators with relatively lower arithmetic intensity, by alleviating the data access bottlenecks effectively.
%For example, since the DIL operator involves larger convolutional windows and data access strides, it is much easier to generate memory-bound programs. With layout optimization, we can alleviate the data access bottleneck effectively.

We achieve similar results on NVIDIA GPU and ARM CPU. Compared with Ansor, \sys achieves an average of $1.5\times$ speedup on NVIDIA GPU (\cref{subfig:exprim_op_cuda}), and $1.4\times$ speedup on ARM CPU (\cref{subfig:exprim_op_android}). We do not include the results of FlexTensor for ARM CPU since it does not support ARM backends. Generally, auto-tuning methods can outperform Torch because non-typical operator configurations are often less optimized in vendor libraries. Further, AutoTVM suffers from small tuning space and FlexTensor has no cost model, thus both demonstrate inferior performance than Ansor and \sys. Additionally, compared with Ansor, \sys can effectively tune data layouts with feedback from operator-level optimization and hence illustrate significant improvements.
% 下面的话没有上下文，逻辑联系不紧，想要表达的意思不清晰
 % Furthermore, it is been long since some templates of AutoTVM were updated (their templates only cover a small set of test cases), thereby performing poorly on many test cases. 

%In summary, \sys outperforms other baselines over all single operator benchmarks, 
% 别找事儿，图上也没看出来
%\textcolor{red}{except for several operator configurations.} For instance, Ansor performs better than \sys on four configurations of T3D on NVIDIA GPU. Ansor exploits a hierarchical search space for loop tuning. We leave such expanding loop tuning space in future work.
%Ansor first generates multiple loop templates and then performs fine-tuning. We notice that some of its searched loop schedules, can locate outside of our loop tuning space. We leave the integration of such multiple-template tuning in the future work.
%Actually, the performance gain brought by layout optimization can be observed from the large margin of performance gap between \sys and FlexTensor, since such two frameworks perform loop optimization only with one similar template for all operators.

% \vspace{-0.02in}
\presub\subsection{End-to-End Benchmark}
\label{subsec:e2e_bench}
%\postsub
% \vspace{-0.02in}

We then evaluate the end-to-end performance of \sys with five neural networks, including applications of 1) image processing: ResNet-18 (R18) \cite{he2016deep}, MobileNet-V2 (MV2) \cite{sandler2018mobilenetv2}, 2) natural language processing: BERT-base (BB) \cite{devlin2018bert}, BERT-tiny (BT) \cite{jiao2019tinybert}, and 3) video processing: ResNet3D-18 (R3D) \cite{hara2017learning}. 
% These network architectures provide popular backbones in many applications. 
For Intel CPU and NVIDIA GPU, the benchmarks use batch sizes of 1 and 16. For ARM CPU, we set the batch size to 1 due to the limited resource.
%Ansor usually uses $NHWO/NDHWO$ because this layout leads to better performance than $NOHW/NODHW$. 

% To verify the effectiveness of the joint tuning and layout propagation, we further define two variants of \sys: (1) \sys-OL, which only involves loop optimization without the joint stage based on default $NHWO/NDHWO$ layouts; (2) \sys-WP, which only eliminates conversion operators between adjacent operators, as that shown in \cref{subfig:layout_prop}. 

% 中文？
For convolutional networks, the input tensor is of shape $N \times 3 \times 224 \times 224$ (image processing) and $N \times 3 \times 16 \times 112 \times 112$ (video processing), respectively. For BERT, the shape of the input tensor is $N \times 128$. For auto-tuning baselines, we set the search budget as 20,000 (which is suggested by Ansor \cite{zheng2020ansor}). We set the budget for the joint stage to 8,000 and the budget for the loop-only stage to 12,000 in \sys. Additionally, Torch uses $NOHW/NODHW$ layouts while AutoTVM and Ansor use $N\frac{O}{o_t}HWo_t/N\frac{O}{o_t}DHWo_t$ after integrating NeoCPU \cite{liu2019optimizing}. 
%Also, the budget for each subgraph is scaled with its amount of computations, \textit{i.e.}, the amount of \textit{floating-point operations} (FLOPs).
% \vspace{-0.1in}


We illustrate the speedup ratio of all methods over Torch in \cref{fig:exprim_network}, where $b1$ denotes batch size 1 and $b16$ denotes batch size 16. The number on top of each bar demonstrates the latency in milliseconds. To verify the effectiveness of the joint tuning and layout propagation, we define two variants of \sys: (1) \sys-OL, which only involves loop optimization without the joint stage based on $NHWO/NDHWO$ layouts; (2) \sys-WP, which only eliminates conversion operators between adjacent operators, as that shown in \cref{subfig:layout_prop}. Compared with Ansor\footnote{Ansor performs better than Torch \cite{paszke2019pytorch} and AutoTVM \cite{chen2018learning}. We omit the results of Torch and AutoTVM due to the lack of space.}, \sys achieves $1.47\times$, $1.39\times$, and $1.46\times$ speedups on Intel CPU, NVIDIA GPU, and ARM CPU, respectively. For R3D, most of its operators are compute-bound, thus \sys achieves similar results with Ansor. For MV2, which is a lightweight network with lower operational intensity, \sys outperforms the baselines significantly. 

%Further, we observe that \sys often exhibits better speedups when the batch size is not large, due to less parallelism and lower operational intensity. Fortunately, small batch sizes are more common in inference scenarios, especially for latency-sensitive applications. 
%In the following, we will further break down the improvements of \sys by benchmarks on \sys-OL and \sys-WP.
%In general, when the batch size is set to 1, the speedup ratios are higher. Also, speedups for convolutional networks are higher than Bert which mainly involves large matrix multiplication operators. With batch size 16, 
%data reuse can be achieved along the batch size dimension which improves the benefits of loop transformation. In the meanwhile, 
%the operational intensity is higher with a large batch size and more operators tend to be compute-bound, which decreases the profits brought by layout optimization. As for matrix multiplication, it is often implemented and optimized at the assembly level in hand-tuning libraries or with low-complexity algorithms (\textit{e.g.}, Strassen algorithm). We observe that \sys just transposes the constant weight tensor in some matrix multiplication operators, or even keep it unchanged on CPU. The transposition optimization is also included in the baselines which further narrows the gaps between \sys. 

Notice that \sys-OL achieves similar performance as Ansor because both of them mainly involve loop tuning. When incorporating layout tuning and basic layout propagation, \sys-WP shows $1.1\times$ speedup over \sys-OL in general and no improvement in a few cases. \sys achieves $1.3\times$ speedup on average compared with \sys-WP. This is because operator fusion is a critical loop-tuning technique to improve performance, while \sys-WP cannot combine layout tuning and loop tuning effectively. 
%For example, the first layer of MV2-b1 contains operators: padding, C2D, bias addition, and ReLU. The C2D in \sys-WP only costs 0.31ms on ARM CPU, but this layer requires 0.52ms in total although other operators involve very few computations. %This is because the loop nest mismatch inhibits operator fusion to promote locality and data bandwidth becomes a new bottleneck accordingly. 
%In contrast, \sys only requires 0.37ms for this layer. %Consequently, the performance gain of \sys compared with baselines is mainly from its layout optimization.


% \vspace{-0.1in}
\presub\subsection{{Micro Benchmark}}
%\postsub
% \vspace{-0.02in}
\label{subsec:micro_bench}

We dive into the details to achieve a better understanding of the system design. First, we present the overhead of layout propagation.
%and show the necessity of introducing constraints in \cref{subsec:layout_prop}. 
We then study the parameter sensitivity of \sys in the end-to-end optimization.
%
%by illustrating the trade-off between final performance, tuning budget, and the search space size. 
%
We will also conduct a case study to help understand the searched layouts and loops. 
%
Finally, we present more observations to provide hints for deep compiler optimization. 
%
Notably, we do not give more experiments on cost model \cite{zheng2020ansor} and the PPO exploration method \cite{ahn2020chameleon} because they are not our major contributions. %We believe more delicate techniques will bring more benefits.

% \subsubsection{Space Pruning:} 
% \begin{figure}
% \centering
% \includegraphics[width=0.46\textwidth]{imgs/layout_tiling_cgpu.pdf} \hfill
% % \vspace{-0.15in}
% \caption{Final reward of different layout tuning templates.}
% \label{fig:layout_tiling}
% \end{figure}
%We first conduct a single-operator micro-benchmark on Kirin 990 SoC. We include three methods for comparison: RL-based exploration for the pruned space with one-level layout tiling templates (denoted as $RL-OT$, $OT$ means one-level tiling), and RL-based exploration but with two-level layout tiling templates (denoted as $RL-TT$), and a random search method with one-level layout tiling templates as the baseline. During exploration, we assess each layout based on \cref{eq:reward_func} after three rounds of loop optimization. The operator we tested is a C2D with $N = 1, O=32, I=3, H=W=226, KH=KW=3$ and stride as 2, which is also the first C2D in network MV2. 

% %We present the results in \cref{subfig:search_speed_bench_v2}. We observe that both the $RL-OT$ and $RL-TT$ methods outperform the random method significantly. As to the search speed, $Random-OT$ shows the fastest search, although the final performance is worse than others. By contrast, $RL-TT$ illustrates the slowest search speed and only outperforms the random method after 550 measurements. Different from them, $RL-OT$ makes a much better trade-off between the search speed and the final performance. With less than 300 measurements, $RL-TT$ can reach 92\% of the final performance, and the latency of which is only three microseconds more than the final performance.

% To evaluate the layout tuning templates, we conduct a micro-benchmark on Intel CPU and NVIDIA GPU. We include three variants for comparison: 1) two-level layout tiling templates; 2) no pruning; 3) one-level layout tiling templates (the default setting). The second variant is achieved by learning to permute with the Sinkhorn method \cite{mena2018learning} for the reorder primitive. We record the best reward found during the layout stage, where the budget is 600 to enable sufficient layout search. As a reference, we take the reward of the NHWI layout as a baseline. We choose ten operators for testing, the first five of them were tested on Intel CPU while the others were tested on NVIDIA GPU. 

% The results are summarized in \cref{fig:layout_tiling}. We observe that one-level layout tiling templates can already reach a similar final performance as the two-level variant. The reward improvement with two-level tiling templates is less than 2\% on average. Moreover, with less than 300 budgets, which is the budget setting in \cref{subsec:single_op_bench}, the exploration with one-level layout tiling templates can reach 94\% of the final reward on average. As to the variant without pruning, over which the one-level tiling improves the reward by 8\% on average. In summary, the one-level tiling achieves a much better trade-off between the final performance and our budget setting.
%However, including the profiling, these results are not applicable to all configurations or platforms. By contrast, the methodology in our case studies could help understanding the optimized layout, and similar analysis can be conducted for other cases

% The results are shown in \cref{fig:exprim_search_speed}. The RLSeqPret method has the fastest search speed which uses only 20\% measurements of other methods. 
% % 
% The RL Walk and RLSeq methods can both achieve similar final performance as RLSeqPret, but with more budgets.
% %
% %These observations are consistent with our expectations since RL often requires massive data to get a better and stabler performance. 
% %
% This is also the reason we pretrain layout RL agents and transfer them to accelerate the automatic search. 
% %
% On the other hand, traditional random search algorithms cannot be easily transferred among tasks. 
% %
% And, the random-walk design of RL also prevents effective pretraining, because it needs much more training data. For example, the reorder actor requires more swaps to obtain the target permutation, and we need to evaluate each layout in the episode by loop optimization to obtain accurate rewards. 
% %
% %Moreover, the search spaces are discrete and lead to challenging combinatorial optimizations. 
% %
% These concerns inspire us to adopt the RLSeqPret method. 

\subsubsection{Layout Propagation Overhead:} 
We here study the overhead of layout propagation to show the necessity of the introduced constraints in \cref{subsec:layout_prop}. We evaluate two subgraphs on 48-core Intel(R) Xeon(R) Gold 5117 CPU @2.0GHz and NVIDIA RTX 3070 GPU. Each subgraph consists of three operators: padding (padding size is 1), C2D ($KH=KW=3, stride=1$), C2D ($KH=KW=1, stride=1$). The input height/width of subgraph\#1 is 7, while it is 14 for subgraph\#2. Besides, all the numbers of input/output channels are 512, except that the number of output channels of the latter C2D ($KH=KW=1$) in subgraph\#2 is 2048. We conduct two variants of \sys: \sys-FP and \sys-BP. \sys-FP will first tune C2D ($KH=KW=3$) and propagate its output layout to the input tensor of the latter C2D ($KH=KW=1$). While \sys-BP will first tune C2D ($KH=KW=1$) and propagate its input layout to the output tensor of the former C2D ($KH=KW=3$). Instead, \sys will tune the two C2Ds separately and insert a layout conversion operator between them according to the third constraint in \cref{subsec:layout_prop}. 

The profiling results are reported in \cref{fig:prop_overhead}, where we use Ansor as a reference point. We observe that \sys outperforms \sys-FP and \sys-WP. In other words, the best output layout of the C2D ($KH=KW=3$) is sub-optimal for the second C2D ($KH=KW=1$), and vice versa. Independent layout tuning for each complex operator brings more benefits while the layout conversion only incurs low overhead (2 microseconds for GPU and 8 microseconds for CPU). Combined with the results of \sys-WP in \cref{fig:exprim_network}, the fusion conflicts incur more overhead than layout conversions when performing layout transformation. We alleviate such two kinds of overheads by layout propagation and eschew the overhead of propagation itself by introducing necessary constraints.


% 这段不太理解，parameter sensitiviry以为看到的是设计引入的参数对性能的影响，但好像不是。此外讨论budget，几乎没见过这种写法。
\subsubsection{Parameter sensitivity:} 
\begin{figure}
	\centering
	\includegraphics[width=0.46\textwidth]{imgs/prop_overhead_cgpu_arxiv.pdf} \hfill
	\caption{The overhead of layout propagation.}
	\vspace{-0.15in}
	\label{fig:prop_overhead}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=0.46\textwidth]{imgs/e2e_layout_tiling_cgpu_v2.pdf} \hfill
	\caption{End-to-end performance of different settings.}
	\vspace{-0.15in}
	\label{fig:search_tradeoff_bench_v2}
\end{figure}

We study the parameter sensitivity by comparing the performance given different budget settings and search space sizes. We include three variants here: 1) two-level tiling templates with 20,000 budget;
%(\textit{i.e.}, 2E4)
2) two-level tiling templates but with 30,000 budget;
%(\textit{i.e.}, 3E4)
3) one-level layout tiling templates with 20,000 budget as the baseline (\textit{i.e.}, same as \cref{subsec:e2e_bench}).

The end-to-end performance in different settings is shown in \cref{fig:search_tradeoff_bench_v2}. The first variant expands the search space size while keeping the budget unchanged. Compared with it, the baseline illustrates 15\% performance improvement on average. By contrast, after setting the budget to 30,000, the second variant improves about 6\% performance over the baseline. Also, more improvements can be obtained if given a larger budget, since one-level tiling templates constitute a subset of the two-level variant. For the budget of 20,000 in \cref{subsec:e2e_bench}, one-level layout tiling templates yield a more effective trade-off between the final performance and the search space size. 
%
The budget of 20,000 to optimize a network typically costs 12-16 hours. But, it is affordable for practitioners as they only need to execute \sys once.
%
%For users who explore new operators, a budget of 1000 can take half to an hour. 
Additionally, these results demonstrate the scalability of the tuning space, which is hard to achieve in prior auto-tuning works.
%
%We further illustrate the trade-off between performance and search budget for end-to-end tuning in \cref{fig:search_tradeoff_bench_v2}. 
%
%In general, a budget of 10000 can already achieve more than 80\% performance. 
%Besides, such trade-off is closely related to the search budget allocation strategy for different subgraphs of a deep model. Thus, the search time could be further reduced by more advanced strategies. Although the budget for each subgraph scales with its floating-point operations in our experiments on \sys, we also provide other optional strategies that can dynamically allocate budgets according to the real-time search results.
%From \cref{fig:exprim_search_speed}, we can also notice that the non-uniform sampling method performs much better than the plain random method in terms of both the final performance and the search speed, which shows the effectiveness of domain knowledge integration during sampling.

% \begin{figure}
% \centering
% \subfigure[Different layouts on Intel CPU.]{\label{subfig:perf_gain_llvm}{\includegraphics[width=0.47\textwidth]{imgs/perf_insight_conv2d_llvm.pdf}}}
% \\
% \subfigure[Different layouts on NVIDIA GPU.]{\label{subfig:perf_gain_cuda}{\includegraphics[width=0.47\textwidth]{imgs/perf_insight_conv2d_cuda.pdf}}}
% \\
% \subfigure[Different layouts on ARM CPU.]{\label{subfig:perf_gain_android}{\includegraphics[width=0.47\textwidth]{imgs/perf_insight_conv2d_android.pdf}}}
% % \vspace{-0.1in}
% \caption{Performance gain of \sys.}
% \label{fig:exprim_perf_gain}
% % \vspace{-0.2in}
% \end{figure}

%\textbf{Performance Gain:} To illustrate the performance gain, we compare \sys with its variant used in \cref{subsec:motiv} which disables layout optimization. This set of experiments is also a supplement to \cref{subsec:motiv} but on the same hardware as those in \cref{subsec:single_op_bench}. Also, we set the search budget to $1000$. The results are shown in \cref{fig:exprim_perf_gain}. On average, \sys improves the performance by 24\%, 22\%, and 27\% when compared with the best one of the three popular layouts on three platforms respectively. However, the optimized layouts for each configuration are different from each other. For instance, on ARM CPU with configuration of $N=8, H=W=230, I=3, O=64, h=w=7, stride=2$ where $h, w$ are the height and the width of the convolutional kernel, and $O$ is the number of output channels, the optimized layout sets the input tensor to $IHNW$, the kernel tensor to $IhwO$, and keep the output tensor as $NOHW$ unchanged. By contrast, changing $h, w$ to $h=w=5$, the optimized layout is $H^\prime NWI H^b$ for the input tensor where $H^\prime$ is the unfolded dimension generated from $H$ and $H^b = 5$ is the block dimension due to unfolding too, $hIwO$ for the kernel tensor, and $NHWO$ for the output tensor. It is worth noting that the input layout in the later case is produced by applying the unfold primitive only once to the the input tensor (the height or the width). Such pattern also arises in the optimization results for other configurations or platforms. We call this special layout \emph{1-step unfold}. Actually, applying the unfold primitive both on the height dimension and on the width dimension rarely appears in optimized layouts. Besides, \sys also rediscovers the spatial pack layout for some configurations. For example, setting $N=1, I=64, H=W=114, O=128, k=w=3, stride=1$, the optimized layout for the input tensor is $NH_0 WIH_1$ where $H_0=19, H_1=6$ are generated by splitting the $H$ dimension with factor 6 (a special case for spatial pack). Besides layout transformation, the performance gain brought by layout propagation is intuitive and will not be evaluated here. 
%It can eliminate another function call at runtime and compared with inserting layout conversion operators directly, which induces more data to write back and load again, such improvement is more significant when a larger amount of data is involved.

\subsubsection{Case study:}
\label{subsubsec:case_study}

% \vspace{-0.1in}
To understand how the joint tuning improves the loop performance, we perform loop optimization based on $NHWO$, $NOHW$, $N\frac{O}{o_t}HWo_t$, and $N\frac{H}{h_t} \frac{W}{w_t} \frac{O}{o_t} h_t w_t o_t$ on Intel CPU. We profiled a small computational graph, which contains several operators: padding (after padding, the tensor will have $N=1, I=3, H=W=230$), C2D ($O=64, KH=KW=7$, convolutional stride is 2), bias addition, and ReLU. This small graph is also the first layer of R18-b1. We set $o_t=16$ for $N\frac{O}{o_t}HWo_t$ ($i_t=3$ for the input tensor), while the searched layout has $h_t = 4, w_t = 16, o_t=16$ for $N\frac{H}{h_t} \frac{W}{w_t} \frac{O}{o_t} h_t w_t o_t$ ($i_t=1$ for the input tensor). {The platform is 48-core Intel(R) Xeon(R) Gold 5117 CPU @2.0GHz.} %不要了吧

\begin{table}[!ht]
	\centering
	\small
	\caption{Profiling results based on several layouts.}
	\begin{tabular}{l@{\hskip 0.1in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c}
		\toprule
		\textbf{Layout (Conv \& Ker)} &\textbf{\#Inst.} &\textbf{\#L1-lds} &\textbf{\#L1-mis}
		&\textbf{\#L1-sts} & \textbf{Lat.}\\
		\midrule
		 $NHWO$ \& $rsIO$& $509.4$ & $166.4$ & $9.7$ & $103.6$ & $0.34$\\
		 \midrule
		 $NOHW$ \& $OIrs$ & $626.9$ & $206.6$ & $4.5$ & $121.3$ & $0.49$\\
         \midrule
		 $N\frac{O}{o_t}HWo_t$ \& $\frac{O}{o_t}\frac{I}{i_t}rsio$& $567.6$ & $193.6$ & $9.9$ & $112.9$ & $0.37$\\
		 \midrule
		 $N\frac{H}{h_t} \frac{W}{w_t} \frac{O}{o_t} h_t w_t o_t$ \& ... & $550.5$ & $174.3$ & $3.9$ & $106.2$ & $0.25$\\
		\bottomrule
	\end{tabular}
	\label{tab:prof_result}
% 	\vspace*{-\baselineskip}
\end{table}

The results are summarized in \cref{tab:prof_result}, where we abbreviate $(KH)(KW)$ to $rs$ for the weight tensor $Ker$. The latency (Lat.) is recorded in milliseconds and others are on a scale of $10^6$. We observe that for all layouts, except $NOHW$, their optimized loop nests prefer reusing input values by computing multiple output channels once with SIMD, thus reporting fewer instructions and fewer cache loads/stores than $NOHW$. Compared with $N\frac{O}{o_t}HWo_t$, $NHWO$ shows better data locality due to the larger tile size for the output channel. Specifically, $O=64$ in $NHWO$ yields a higher reuse rate than $o_t=16$ in $N\frac{O}{o_t}HWo_t$, as analyzed in \cref{subsec:space_build}. Further, $N\frac{H}{h_t} \frac{W}{w_t} \frac{O}{o_t} h_t w_t o_t$ achieves more efficient cache utilization  (only $2\%$ misses) than $NHWO$, due to the contiguous storage of intra-tile data elements after layout tiling.

%However, this incurs many writes for the output tensor for $NHWI$, because it cannot stage all intermediate values in registers (more stores in \cref{tab:prof_result}). In contrast, both $N\frac{I}{i}H^\prime W^\prime h^\prime w^\prime i$ and $N\frac{I}{i}HWi$ can alleviate this overhead via the tiling on input channels. Further compared with $N\frac{I}{x}HWx$, $N\frac{I}{i}H^\prime W^\prime h^\prime w^\prime i$ can access the tile $h^\prime w^\prime i$ with much less cache misses, because the elements are stored in memory contiguously after layout tiling.
%Further, the interleaved instructions also compute several positions along the spatial dimensions of the output tensor with a single input value (the sliding-window pattern has overlaps naturally). However, this then lead to more register shuffle instructions to align the input values (more instructions in \cref{tab:prof_result}). 
%While the $N\frac{I}{x}H^\prime W^\prime h^\prime w^\prime x$ prefers vector multiplications along $w$ and $w^\prime$. However, there exists poor locality on the boundaries for $N\frac{I}{x}\frac{H}{h}\frac{W}{w}xhw$. 

%Note that accesses on boundary will happen repeatedly due to the $O\times I$ channels (more cache misses in \cref{tab:prof_result}). 
% By contrast, the vector multiplications in the $N\frac{I}{x}n_h n_w x h^\prime w^\prime$ case present temporal locality on the weight tensor (multiplications along $w^\prime$ require the same weight values), hence demanding less bandwidth, and achieve spatial locality on the input tensor (continuous accesses). 
% , because the layout performance is sensitive to the settings and there are no panacea for layouts. 
% For example, the searched layouts for C2D\textit{s} on GPU include various reorders and are hard to summarize regular patterns. 
% However, such case study could help understanding the optimized layout, while similar analysis can be conducted for other cases. 

%We profile three C2D operators with different input and kernel configurations: 
% \begin{enumerate}
%     \item $H=W=114, h=w=3, STRIDE=1$, 
%     \item $H=W=116, h=w=5, STRIDE=2$, 
%     \item $H=W=118, h=w=7, STRIDE=2$.
% \end{enumerate} 
% Besides, we set $N=1,\,I=64,\,O=128$ for all three configurations.
% \cref{tab:prof_result} shows the results where we record the number of instructions $\#Inst.$, the number of L1 data cache related events, and the latency in milliseconds ($Lat.$). The layouts of the input tensor are $NH^\prime WIH^b$, $NH^\prime IWH^b$, and $NWH^\prime H^bI$ for $\mathcal{X}_1$, $\mathcal{X}_2$, and $\mathcal{X}_3$, respectively. The layouts of the kernel tensor are $wIhO$, $whIO$, and $whIO$, while the output layouts are all $NHWO$. Except for the latency column, the numbers before and after the symbol $/$ are the results on a scale of $10^7$ for 1-step unfold layout and $NIHW$ layout respectively. Note that the computational cost of the second configuration is smaller than that of the first one. However, it is hard to get a shorter latency with the $NIHW$ layout (3.5ms v.s. 2.6ms). Unlike the spatial pack layout which improves the performance mainly by decreasing cache miss rate, we notice that 1-step unfold can reduce the number of cache loads effectively. Also in the later two rows, the numbers of instructions for 1-step unfold are much less than those of $NIHW$. With unfolding, we can better exploit SIMD instructions because the unfolded dimension is continuous. Furthermore, this leads to more efficient utilization of registers, thus less cache references. Besides, unfolding two dimensions of the input tensor will cause aggressive data expansion, increasing data movements in the layout conversion operator. By contrast, 1-step unfold strikes a balance between the performance improvement and the overhead of layout conversion. The optimized results for GPUs are more complicated and hard to discover regular patterns. Some layouts are obtained just by reordering the dimensions. 1-step unfold also appears but not that common. 

% 大长句，理解不明白。 此外这里对深入理解又显得太浅了
\subsubsection{Other observations:} {Besides the profiled results, we observe that the $o_t$ parameter in the templates to tile output channels is often tuned as twice as the number of vector lanes that the platform supports when the spatial dimensions are not tiled.} Specifically, we observe that $o_t=32$ on Intel CPU, $o_t=8$ on NVIDIA GPU, and $o_t=8$ on ARM CPU frequently arise, although the number of vector lanes with float32 data types is 16 for AVX-512, 4 for CUDA, and 4 for NEON. This is different from many hand-tuned libraries. However, these results are not applicable to all configurations or platforms. By contrast, the methodology in our micro-benchmarks could help understand the optimized layout, and similar analysis can be conducted for other cases.

==> secs/graph_sch.tex <==
\presec\section{Graph Scheduler}\postsec

End-to-end optimization for a computational graph leads to combinatorial explosion of the search space, thus we design a graph partition submodule which partitions a graph into relatively independent subgraphs that can be optimized in parallel to speedup the search. In addition, we also include a layout propagation submodule to refrain the number of layout conversion operators to reduce the runtime overhead.

%End-to-end optimization for a computational graph leads to further expansion of the search space, hence placing all operators and tensors in a shared space will induce unbearable search time. 

\presub\subsection{Graph Partition}\postsub
A computational graph can be expressed as $G = (V, E)$ where $V$ is the set of nodes representing operators, $E$ is the set of edges denoting tensors. Graph partitioning is to split $G$ into disjoint subgraphs $G_0=(V_0, E_0), G_1=(V_1, E_1), ..., G_{n-1}=(V_{n-1}, E_{n-1})$. Since subgraphs are optimized in parallel, the search time $t^s(\cdot)$ is:
\begin{align}
	t^s(G) = \max_{i\in\{0, 1, ..., n-1\}}{t^s(G_i)}\, .
\end{align}

Unlike critical path based graph partitioning \cite{mayer2017tensorflow, qararyah2020computational, zhang2020efficient, ding2020ios} which oftentimes aims at optimizing the inference where subgraphs will be deployed in different devices, our graph partitioning is only performed during compilation. Consequently, we partition the graph following a topological order, and the execution time $t^r(\cdot)$ after searching can be calculated as:
\begin{align}
	t^r(G) = \sum_{i=0}^{n-1}(t^r(G_i))\, .
\end{align}

We formulate the graph partitioning as an optimization problem by considering both the execution time and the search time:
\begin{align}
	& \min t^r(G) + \lambda t^s(G) \nonumber \\
	\Leftrightarrow & \min \sum_{i=0}^{n-1}(t^r(G_i)) + \lambda \max_{i\in\{0, 1, ..., n-1\}}{t^s(G_i)} \, ,
	\label{eq:min_gp_1}
\end{align} where $\lambda$ is a constant denoting the weight of search time.

Since graph partitioning is performed before search, it is difficult to estimate both $t^r$ and $t^s$. To this end, we first split the total search time into a finite sequence of time units $t_0, t_1, ..., t_m$ and the running time of $G_i$ at $t_j$ where $j < m$ is $t^r_j(G_i)$. If $m$ is large enough, we can obtain the optimal execution time $t^r_m(G_i)$ by exhaustive search. We denote this optimal time as $t^\star(G_i)$ which is the theoretical lower bound of $t^r(G_i)$ and keep unchanged given $G_i$. Thus \cref{eq:min_gp_1} is equivalent to:
\begin{align}
	\min \sum_{i=0}^{n-1}((t^r - t^\star)(G_i)) + \lambda \max_{i\in\{0, 1, ..., n-1\}}{t^s(G_i)} \, .
	\label{eq:min_gp_2}
\end{align} 
In addition, we assume $t^r_m(G_i) = \frac{t^r_{m-1}(G_i)}{1 + \beta(G_i)}$ which means we can decrease the execution time $t^r(G_i)$ by a ratio of $1 + \beta(G_i)$ with each unit-time search. $\beta(\cdot)$ is determined specific $G_i$ and the larger $\beta(\cdot)$ is, the shorter the search time will be. Then minimizing the search time can be estimated by minimizing $-\beta(\cdot)$.

Although the assumption on $\beta$ is strong, the relative value of $\beta$ for different subgraphs is more important.
Then the optimization goal can be transformed to:
\begin{align}
	&\min \sum_{i=0}^{n-1}((t^r - t^\star)(G_i)) - \lambda \max_{i\in\{0, 1, ..., n-1\}}\beta(G_i)\, ,
	\label{eq:min_gp_3}
\end{align}.

Note that $t^r - t^\star$ is the gap between the execution time after searching and its lower bound and can be viewed as a measure of difficulty on optimizing $G_i$. Although directly calculating $t^r$ is hard, we can approximate $t^r - t^\star$ by $t^r_0 - t^r_1$ because generally, $t^r_0 - t^r_1$ is also a measure of difficulty on search. Then \cref{eq:min_gp_3} can be estimated by sampling (performing only one round of search for each subgraph) to obtain $t^r_1(G_i), t^r_0(G_i)$ and $\beta(G_i) = \frac{t^r_0}{t^r_1} - 1$.

\begin{figure}
	\centering
	\includegraphics[width=0.15\textwidth]{imgs/cyclic_graph_partition.pdf}
	\caption{Cyclic dependency between subgraphs.}
	\label{fig:cyclic_gp}
\end{figure}

With \cref{eq:min_gp_3}, our graph partitioning mainly consists of three steps: (\romannum{1}) sort the operators in topological order and generate all candidates of graph partitioning; (\romannum{2}) drop those candidates involving cyclic dependencies, such as the partition scheme in \cref{fig:cyclic_gp}; (\romannum{3}) evaluate \cref{eq:min_gp_3} on all candidates and select the best.

\subsection{Layout Propagation}

\begin{figure}
	\centering
	\includegraphics[width=0.35\textwidth]{imgs/conv_comp_graph.pdf}
	\caption{Computational graph with two operators.}
	\label{fig:conv_comp_graph}
\end{figure}

\begin{figure}
	\centering
	\begin{subfigure}{0.4\textwidth}
		\centering
		\includegraphics[width=\linewidth]{imgs/layout_conversion.pdf}
		\caption{Layout conversion operator.}
		\label{subfig:layout_conversion_op}
	\end{subfigure}
	~
	\begin{subfigure}{0.26\textwidth}
		\centering
		\includegraphics[width=\linewidth]{imgs/layout_prop.pdf}
		\caption{Layout propagation.}
		\label{subfig:layout_prop}
	\end{subfigure}
	\label{fig:layout_conversion}
	\caption{Two ways to achieve runtime layout conversion.}
\end{figure}

Our layout propagation submodule is used to refrain layout conversion operators and extended to prune the search space. Provided a computational graph in \cref{fig:conv_comp_graph}, if C2D requires a different layout $\mathcal{X^\prime}$, it can be achieved by two ways: (\romannum{1}) insert a conversion operator as shown in \cref{subfig:layout_conversion_op}; (\romannum{2}) let the padding operator yields each element based on the new layout directly as in \cref{subfig:layout_prop}. The second way, which is called layout propagation, lifts the optimization for the C2D operator up to graph level since it also influences the performance of the padding operator.

\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth]{imgs/layout_prop_bijective.pdf}
	\caption{Layout propagation across multiple bijective operators.}
	\label{fig:layout_prop_bijective}
\end{figure}

On the other hand, \emph{bijective} operators (there exists an one-to-one mapping between one of its input tensors and the output tensor), such as element-wise-add operator (EwAdd) and ReLU operator, are insensitive to layout transformation and we can prune the search space by skipping such operators for layout optimization. For instance, given a computation graph in \cref{fig:layout_prop_bijective}, the input layout of $C2D$ can be propagated forward along the path $C2D \rightarrow ReLU \rightarrow EwAdd \rightarrow padding$. In other words, we skip two bijective operators and the layout search only involves one tensor on this path. Actually, the resulting graph is equivalent to \cref{subfig:layout_prop} on layout optimization. Such propagation is also achieved through primitives. For example, if we have searched a sequence of layout primitives for the input tensor of $C2D$, we duplicate this sequence to the output and the input of $ReLU$, so as to $EwAdd$ and finally the output of $padding$.

Unfortunately, there are always exceptions. First, one-to-many layout transformation induces data expansion and propagating them to other operators will lead to redundant computation. Second, some operators, such as padding, are insensitive to layout as well but not bijective and we cannot pass primitives through such operators because the shapes of its input and output are inconsistent.

Consequently, we first generate a coarse-grain propagation plan for each subgraph after graph partitioning and refine it during search. Specifically, we first sort the operators in each subgraph following reversed topological order. Then we analyze each subgraph and mark some of the operators as bijective. During search, the layout of some input tensor of a non-bijective operator can be propagated forward along a path until another non-bijective operator or the start node of a subgraph. Also, the output layout of the last non-bijective operator will also be propagated backward until the last node of this subgraph. Then if the searched primitives contains one-to-many transformation, we insert a conversion operator right before the non-bijective operator. In this case, the layouts along the original propagation path will keep untouched. When the search for all subgraphs completes, we perform a post processing which inserts conversion operators among subgraphs if needed, and then fuses all conversion operators intra- and inter- subgraphs with its previous operator to further reduce the runtime overhead of layout conversion.

% 加到哪里
%\textbf{Named Dimension.} Before illustrating layout propagation, we first describe a submodule \emph{named dimension} which allows layout analysis among various operators and tensors. Named dimension is to assign an explicit identifier, such as a symbol or a string, to the dimensions of a tensor. For instance, given a 3-D tensor with shape $M \times N \times K$, we can use three variables $M\_nd, N\_nd, K\_nd$ rather than just indexes $0, 1, 2$ to identify the three dimensions. This technique improves the code readability and make the analysis of compiler easier because named dimension can be a special structure which contains more information. Named dimension for tensor has been advocated by several works [CITE]. Till now, we have seen its application in Tensor Comprehension framework but only as syntactic sugar. In \sys, we extend named dimension to achieve layout propagation between different tensors and operators.

%The transformation of shape and index in the above primitives only adjusts the accessing order, the actual storage of elements in a tensor has not been altered. For constant tensors, we can change the storage at compiling stage. Nonetheless, tensors output by other operators require runtime transformation. For instance, assuming we have two C2D operators as shown in [Fig] where an operator performs convolution on the output of another. The kernel tensors of each C2D operator form a constant tensor. Layout primitives applied on constant tensors will not induce runtime overhead to perform physical storage reorganization. However, if we find a data layout $NIHW$ for the input of the second C2D while the first C2D still outputs $NHWI$, we have two ways to achieve the physical data transformation: (\romannum{1}) insert an explicit data transformation operator between the two C2Ds; (\romannum{2}) change the output layout of the first C2D to $NIHW$ either. Changing the output layout of the first C2D is referred as layout propagation in traditional compiler field but we will extend its concept later.
%
%Both methods have obvious advantages and disadvantages. Introducing an data transformation operator brings explicit runtime overhead, while the layout propagation may result in a suboptimal output layout for the previous C2D. However, optimizing the data transformation operator is also easy to handle. We can fuse it with the former operator to avoid that writing all data back and reading them again. To achieve the layout propagation, the optimization for the input layout of the second operator is not local anymore, because it will affect the performance of other operators.
%
%We design a few heuristics to determine which method to use for a computational graph.

%-------------------------------------------------------------------------------

==> secs/sys_overview.tex <==
\presec\section{Design Overview}\postsec
\begin{figure}[!ht]
	\centering
	\includegraphics[width=0.47\textwidth]{imgs/overview_v2.pdf}\hfill
% 	\vspace{-0.1in}
	\caption{Design overview of \sys.}
	\label{fig:design_overview}
% 	\vspace{-0.15in}
\end{figure}

The system overview of \sys is illustrated in \cref{fig:design_overview}.

First, the developer provides an algorithm description of the deep learning model. 
%
%Then, the graph scheduler partitions the original computational graph into several subgraphs where each subgraph contains multiple operators. 
%
%The graph scheduler then extracts layout tasks and graph tasks and allocates search budgets to them.
%The graph scheduler then produces a coarse-grain layout propagation plan which indicates the set of tensors to optimize for each subgraph. 

Second, the automation module extracts various layout tasks and graph tasks from the computational graph. Then for each task, it encodes the involved tensors and operators as a point in its search space. 
%
Next, it exploits reinforcement learning to explore the searching space and uses a cost model as a reference to avoid compilation and evaluation for each step. 
%
When the exploration completes, it decodes the best point found in the search space into a sequence of layout and loop primitives guided by general templates. 

Third, the infrastructure module applies those primitives to perform loop transformation and layout transformation by altering the data layouts of tensors and rewriting their accessing expressions to generate an optimized \emph{intermediate representation} (IR). 
%
Finally, we translate this IR to executable codes on different hardware platforms.

